Valid Text-to-SQL Generation with Unification-based DeepStochLog

Large language models have been used to translate natural language questions to SQL queries. Without hard constraints on syntax and database schema, they occasionally produce invalid queries that are not executable. These failures limit the usage of these systems in real-life scenarios. We propose a neurosymbolic framework that imposes SQL syntax and schema constraints with unification-based definite clause grammars and thus guarantees the generation of valid queries. Our framework also builds a bi-directional interface to language models to leverage their natural language understanding abilities. The evaluation results on a subset of SQL grammars show that all our output queries are valid. This work is the first step towards extending language models with unification-based grammars. We demonstrate this extension enhances the validity, execution accuracy, and ground truth alignment of the underlying language model by a large margin. Our code is available at https://github.com/ML-KULeuven/deepstochlog-lm.

==> method_v0.tex <==
\section{Methodology}

As shown in Figure \ref{fig:workflow}, our logic program written in Prolog has three parts: facts, rules, and a query. The facts are automatically generated from $S$ of $db$, describing the associations between $db$, $T$, and $C$. The Prolog query takes the form $query(nl, db, Q)$, where $Q$ is a tokenized list of the ground truth $q$. $Q$ is known in training and masked by the wildcard symbol "\_" in evaluation. The rules contain predicate expressions that denote relationships among facts with logical implications (:-). They also cover NDCG rules which are illustrated in section \ref{sec:deepstochlog}. In section \ref{sec:inflearn}, we present inference and learning processes in our framework.

\subsection{DeepStochLog (NDCGs)} \label{sec:deepstochlog}

A CFG defines a set of rewriting rules of the form $V \rightarrow W_1, ..., W_n$, where $V$ is a non-terminal and $W_i$ is either a terminal or a non-terminal. DCGs are a popular logic-programming-based extension of CFGs \cite{pereira1980definite} that can be executed as Prolog programs. They replace non-terminals in CFGs by logical atoms $a(l_1, .., l_n)$ with a predicate $a$ and $n$ terms $l_i$. A term is a constant, a logical variable, or a structured term $f(l_1, ..., l_n)$ where f is a functor. DCG rules take the format $nt\rightarrow  g_1, ..., g_n$, where $nt$ is a logical atom, a goal $g_1, ..., g_n$ is a sequence and $g_i$ in the sequence is a logical atom or a list of terminals and logical variables. DCGs are unification-based and can represent context-sensitive languages. Moreover, they allow queries and operations to Prolog predicates between curly brackets to apply further constraints and computations in inference. This property makes DCGs even more expressive. We refer to \cite{flach1994simply, sterling1994art} for more information on DCGs.

In example \ref{ex:cfgdcg}, we show the difference between CFGs (commonly used in previous grammar-based studies) and DCGs (used by us) in generating basic SQL queries on the dog kennels database in Figure \ref{fig:workflow}. The CFG with limited expressiveness cannot represent relationships between tables and columns. The column domain is defined as all columns in the database. It can lead to invalid queries mismatching tables and columns, for example, "SELECT treat\_id FROM Dogs". The DCG avoids this error and respects the database schema by bounding the column domain to columns in a specific table. Example \ref{ex:cfgdcg} demonstrates DCGs can provide syntax guarantee, schema guarantee, and thus valid guarantee for SQL query generation. 

\begin{example}%
\label{ex:cfgdcg}
\small
A CFG (a) and a similar DCG (b).\\

\vspace{-8mm}
\begin{minipage}[t]{.8\linewidth}
\begin{align*}
    a)&\ T \rightarrow \textnormal{"Dogs",\ "Professionals",\ ‘Treatments“}\\
    &\ C \rightarrow \textnormal{"dog\_id",\ ...,\ "abandoned\_yn",\ "prof\_id",\ ...,\ "role\_code",\ "treat\_id",\ ...,\ "type\_code"}\\
    &\ Q \rightarrow \textnormal{"SELECT"}\  C\ \textnormal{"FROM"}\ T
\end{align*}
\end{minipage}

\begin{minipage}[t]{.43\linewidth}
    \begin{align*}
        b)&\ table(\textnormal{"Dogs"}) \rightarrow \textnormal{"Dogs"}\\
        &\ table(\textnormal{"Professionals"}) \rightarrow \textnormal{"Professionals"}\\
        &\ table(\textnormal{"Treatments")} \rightarrow \textnormal{"Treatments"}
    \end{align*}
  \end{minipage}
  \begin{minipage}[t]{.55\linewidth}
\begin{align*}
&column(\textnormal{"Dogs"}) \rightarrow \textnormal{"dog\_id",\ ...,\ "abandoned\_yn"}\\
&column(\textnormal{"Professionals"}) \rightarrow \textnormal{"prof\_id",\ ...,\ "role\_code"}\\
&column(\textnormal{"Treatments"}) \rightarrow \textnormal{"treat\_id",\ ...,\ "type\_code"}
\end{align*}
 \end{minipage}

\vspace{-4mm}
\begin{minipage}[t]{.52\linewidth}
\begin{align*}
    &\ Q \rightarrow \textnormal{"SELECT"}\  column(T)\ \textnormal{"FROM"}\ table(T)
\end{align*}
\end{minipage}
    
\end{example}

An SDCG adds probabilities to the DCG rules with the form $p_i:: nt\rightarrow  g_1, ..., g_n$. For the rules of the same non-terminal predicates, SDCGs require their probabilities to sum to 1. They define a probability distribution over possible parses of a sequence, which allows the most likely parse to be determined. In Figure \ref{fig:workflow}, $p_i$ is omitted when it equals 1.0.

DeepStochLog further extends SDCGs to NDCGs that integrate neural networks. An NDCG rule takes the format 
\begin{displaymath}
  nn( m,[I_1, ... , I_X],[O_1, ... ,O_Y],[D_1, ... , D_Y]) :: nt \rightarrow  g_1, ... , g_n.
\end{displaymath}
It is equivalent to the expression with curly brackets in Figure \ref{fig:workflow}. The $nn$ predicate denotes a neural network $m$ that tasks input variables $I_1, ..., I_X$ and outputs a probability distribution over variables $O_1, ... ,O_Y$ with domains $D_1, ... ,D_Y$ respectively. Thus, each substitution $\sigma$ of the input variables is mapped to a set of output substitutions $\theta_j$ with a probability $p_j$. 

For example, consider the rule "$table(NL, DB, T) \rightarrow \{nn(table\_nn, [NL], T), database \newline (DB, Tables), domain(T, Tables)\}, [].$" in Figure \ref{fig:workflow}. The neural network $table\_nn$ receives the natural language sentence $NL$ and returns a probability for each of the three possible tables: Dogs, Professionals, and Treatments. The probabilities indicate how likely $NL$ queries on each table. Given the input substitution $\sigma = \{NL = \textnormal{`Find the ids of professionals who have ever treated dogs.'}\}$, $table\_nn$ could produce the output substitutions $\theta_0 = \{T = \textnormal{"Dogs"}\}; \theta_1 = \{T = \textnormal{"Professionals"}\}; \theta_2 = \{T = \textnormal{"Treatments"}\};$ with probabilities 0.2; 0.2; 0.6. Thus, the NDCG rule represents a set of grammar rules: $0.2:: table(\textnormal{"Find ... dogs.", "dog\_kennels", "Dogs"});  0.2:: table(\textnormal{"Find ... dogs.", "dog\_kennels", "Professionals"});  0.6:: table(\textnormal{"Find ... dogs.", "dog\_kennels",} \newline \textnormal{ "Treatments"})$. Here, we apply the empty production. The rule produces the empty sequence but retrieves the table variable $T$ substitutions, which helps determine the column domain in the column rule through the Prolog unification mechanism. Unlike the autoregressive models, the empty production allows us to deal with tables before columns which better fits human intuitions. 


\subsection{Inference and Learning} \label{sec:inflearn}

\paragraph{Inference} The inference process in our framework computes the probability $P(derives(G))$ for a goal $G=query(nl, db, Q)$, given a DeepStochLog program, a natural language sentence $nl$, a database $db$ and a (possibly unknown) tokenized SQL query sequence $Q$. It involves two steps, a logical inference and a probabilistic one. 

The logical inference uses resolution to find all possible answers for $G$, i.e. derivations $d(G\theta)$ that result in the terminal sequence $Q$ with answer substitution $\theta$. Figure \ref{fig:inference} shows an SLD resolution tree (a) and the AND-OR circuit translated from it for the probability inference (b). Follow DeepStochLog \cite{winters2022deepstochlog}, we use SLG resolution with tabling \cite{chen1996tabled} to prove the same interim goals once and reduce inference time. 

\begin{figure} 
  \centering
  \includegraphics[width=\linewidth]{inference v1.jpg}
  \caption{Inference steps on a text-to-SQL instance.}
  \label{fig:inference}
\end{figure}

The probabilistic inference calculates $P(derives(G))=\sum_{d(G\theta)=Q}\prod_{r_i \in d(G\theta)}p_i^{k_i}$, where $p_i$ is the probability of the rule $r_i$ used for $k_i$ times in the derivation. This computation equals a bottom-up evaluation of the AND-OR circuit that compiles the logical circuit to an arithmetic circuit with the $(+, \times)$ semiring \cite{kimmig2011algebraic} (substitute the AND-nodes by multiplications and OR-nodes by summations). Similarly, The most probable derivation for $G$ is identified with the $(\max, \times)$ semiring. 

\paragraph{Learning}

Consider a dataset $D={(G_i\theta_i, Q_i)}$, where a goal $G_i = query(nl_i, db_i, Q_i)$, $\theta_i$ is a substitution for $G_i$ and $Q_i$ is a tokenized SQL sequence. All samples in the dataset are positive ones with a probability of 1.0. Learning in our framework with the negative log-likelihood loss function is defined as the following optimization problem over the vector $p$ of rule probabilities:
\begin{equation}
\label{eq:learning}
    \min_{p} \sum\nolimits_{(G_i\theta_i, Q_i) \in D} -log(P(derives(G_i\theta_i,Q_i);p))
\end{equation}
Thanks to the arithmetic circuit, our framework can be trained end-to-end with a differentiable computational graph. The gradients w.r.t $p$ can be calculated automatically and be backpropagated to the neural networks seamlessly to train their internal parameters. 

Moreover, in this text-to-SQL task, only one derivation is possible when $Q_i$ is known during training. Hence,
\begin{displaymath}
\begin{aligned}
     (\ref{eq:learning}) &= \min_{p} \sum\nolimits_{(G_i\theta_i, Q_i) \in D} -log(\prod\nolimits_{r_j \in d(G_i\theta_i)=Q_i}p_j^{k_j}) \\
     &= \sum\nolimits_{(G_i\theta_i, Q_i) \in D} \sum\nolimits_{r_j \in d(G_i\theta_i)=Q_i} \min_{p_j} -k_jlogp_j
\end{aligned}
\end{displaymath}
We are allowed to train the neural networks separately in a supervised manner as all the intermediate goals are observable. 
